Two Constraint Compilation Methods for Lifted Planning

We study planning in a fragment of PDDL with qualitative state-trajectory constraints, capturing safety requirements, task ordering conditions, and intermediate sub-goals commonly found in real-world problems. A prominent approach to tackle such problems is to compile their constraints away, leading to a problem that is supported by state-of-the-art planners. Unfortunately, existing compilers do not scale on problems with a large number of objects and high-arity actions, as they necessitate grounding the problem before compilation. To address this issue, we propose two methods for compiling away constraints without grounding, making them suitable for large-scale planning problems. We prove the correctness of our compilers and outline their worst-case time complexity. Moreover, we present a reproducible empirical evaluation on the domains used in the latest International Planning Competition. Our results demonstrate that our methods are efficient and produce planning specifications that are orders of magnitude more succinct than the ones produced by compilers that ground the domain, while remaining competitive when used for planning with a state-of-the-art planner.

==> figures/cactus/legend_symk_compilers.tex <==
\begin{tikzpicture}
    \begin{customlegend}[legend entries={\lccr{+}\symk,\lcc{+}\symk,TCORE{+}\symk}, legend columns=-1, legend style = {draw=none, font=\footnotesize}]
        \addlegendimage{bblue, solid, thick, mark=none}
        \addlegendimage{rred, solid, thick, mark=none}
        \addlegendimage{ggreen, solid, thick, mark=none}
    \end{customlegend}
\end{tikzpicture}

==> figures/cactus/symk_time_grd.tex <==
\begin{tikzpicture}[scale=1.15]
\begin{axis}[
    ymode=log,
    xlabel={Number of Solved Instances},
   ylabel={Execution Time (sec)},
    title= Ground Constraints,
    width=4.2cm,
    height=4.2cm,
    xmax=150,
    xtick={0, 70, 140},
    ymax=32523,
     ymin=0.2,
    ytickten={-1, ..., 5},
     minor y tick num=9,
     xlabel style={yshift=3pt},
     ylabel style={yshift=-3pt},
     title style={yshift=-5pt},
     font=\scriptsize,
]
\addplot+ [
sharp plot,
color=bblue,
solid, thick,
mark=none,
] table[
row sep=\\]{
0 0.1 \\
1 0.41979 \\
2 0.89476 \\
3 1.37345 \\
4 1.88875 \\
5 2.4232299999999998 \\
6 3.1031899999999997 \\
7 3.8267799999999994 \\
8 4.56178 \\
9 5.32593 \\
10 6.14325 \\
11 7.25035 \\
12 8.36984 \\
13 10.08003 \\
14 12.001100000000001 \\
15 13.92932 \\
16 16.27591 \\
17 18.74863 \\
18 21.281489999999998 \\
19 24.055099999999996 \\
20 26.887449999999994 \\
21 29.720069999999993 \\
22 32.84316999999999 \\
23 36.50616999999999 \\
24 40.40249999999999 \\
25 44.40237999999999 \\
26 48.667419999999986 \\
27 53.813999999999986 \\
28 59.228929999999984 \\
29 65.39178999999999 \\
30 72.54899999999999 \\
31 81.39616 \\
32 91.38462 \\
33 101.48186 \\
34 115.2905 \\
35 129.35604 \\
36 145.43282 \\
37 163.8999 \\
38 184.17835 \\
39 207.70116 \\
40 232.22447 \\
41 257.25389 \\
42 287.66512 \\
43 323.82714 \\
44 362.23053 \\
45 401.05748 \\
46 440.45685 \\
47 480.2761 \\
48 523.14651 \\
49 568.85481 \\
50 617.3532200000001 \\
51 669.85414 \\
52 724.6163200000001 \\
53 782.25134 \\
54 841.73548 \\
55 916.54614 \\
56 996.36009 \\
57 1078.40024 \\
58 1161.28279 \\
59 1264.64498 \\
60 1441.91172 \\
61 1695.43063 \\
62 1979.69053 \\
63 2301.99066 \\
64 2646.9597599999997 \\
65 3007.04672 \\
66 3513.29753 \\
67 4235.184499999999 \\
68 5069.440809999999 \\
69 5998.134899999999 \\
70 7243.984519999999 \\
};

\addplot+ [
sharp plot,
color=rred,
solid, thick,
mark=none,
] table[
row sep=\\]{
0 0.1 \\
1 0.43139 \\
2 0.8841399999999999 \\
3 1.3860899999999998 \\
4 1.8970099999999999 \\
5 2.41789 \\
6 3.05108 \\
7 3.72227 \\
8 4.51402 \\
9 5.3655800000000005 \\
10 6.25858 \\
11 7.18006 \\
12 8.14325 \\
13 9.16614 \\
14 10.287700000000001 \\
15 12.21874 \\
16 14.26993 \\
17 16.54084 \\
18 18.94263 \\
19 21.36374 \\
20 23.80544 \\
21 26.31715 \\
22 29.07892 \\
23 31.84996 \\
24 35.13158 \\
25 38.90241 \\
26 42.69333 \\
27 48.01435 \\
28 53.42536 \\
29 59.146559999999994 \\
30 65.24740999999999 \\
31 72.31920999999998 \\
32 79.60024999999999 \\
33 88.28118999999998 \\
34 99.05258999999998 \\
35 110.03361999999998 \\
36 121.48456999999999 \\
37 134.18569 \\
38 146.93680999999998 \\
39 160.69801999999999 \\
40 174.59894999999997 \\
41 198.48991999999998 \\
42 229.78100999999998 \\
43 261.95196999999996 \\
44 297.57350999999994 \\
45 333.88521999999995 \\
46 370.32635999999997 \\
47 411.92722999999995 \\
48 453.7881699999999 \\
49 495.67072999999993 \\
50 539.05329 \\
51 583.2449399999999 \\
52 627.44724 \\
53 671.73897 \\
54 717.08237 \\
55 765.15333 \\
56 857.23668 \\
57 952.1176899999999 \\
58 1047.87862 \\
59 1147.95176 \\
60 1251.6728699999999 \\
61 1395.73444 \\
62 1690.84586 \\
63 2020.12962 \\
64 2408.48151 \\
65 2812.38917 \\
66 3450.63359 \\
67 4292.81446 \\
68 5228.87104 \\
69 6594.37274 \\
};

\addplot+ [
sharp plot,
color=ggreen,
solid, thick,
mark=none,
] table[
row sep=\\]{
0 0.1 \\
1 4.1243 \\
2 15.10059 \\
3 28.03164 \\
4 41.32551 \\
5 54.76972 \\
6 68.58037 \\
7 85.21983 \\
8 102.22707 \\
9 121.62688 \\
10 141.57565 \\
11 164.76636 \\
12 209.94018999999997 \\
13 267.58608999999996 \\
14 329.98088999999993 \\
15 406.0039099999999 \\
16 483.63240999999994 \\
17 571.58733 \\
18 662.8837799999999 \\
19 757.9816199999999 \\
20 858.2068099999999 \\
21 962.3592899999999 \\
22 1080.08892 \\
23 1234.2463699999998 \\
24 1401.8015799999998 \\
25 1577.30046 \\
26 1756.24877 \\
27 1935.6632399999999 \\
28 2242.8102 \\
29 2556.75212 \\
30 2887.77284 \\
31 3273.16557 \\
32 3706.62738 \\
33 4158.9762599999995 \\
34 4643.201179999999 \\
35 5151.635089999999 \\
36 5660.446759999999 \\
37 6180.839689999999 \\
38 6827.379339999999 \\
39 7630.333929999999 \\
40 8501.520129999999 \\
41 9573.32383 \\
42 10841.987669999999 \\
};

\end{axis}
\end{tikzpicture}


==> figures/cactus/symk_time_lfd.tex <==
\begin{tikzpicture}[scale=1.15]
\begin{axis}[
    ymode=log,
    xlabel={Number of Solved Instances},
    title= Non-Ground Constraints,
    yticklabels={},
    width=4.2cm,
    height=4.2cm,
    xmax=150,
    xtick={0, 70, 140},
    ymax=47514,
     ymin=0.2,
    ytickten={-1, ..., 5},
     minor y tick num=9,
     xlabel style={yshift=3pt},
     ylabel style={yshift=-3pt},
     title style={yshift=-5pt},
     font=\scriptsize,
]
\addplot+ [
sharp plot,
color=bblue,
solid, thick,
mark=none,
] table[
row sep=\\]{
0 0.1 \\
1 0.50814 \\
2 1.0590100000000002 \\
3 1.9684600000000003 \\
4 2.9983500000000003 \\
5 4.06616 \\
6 5.13887 \\
7 6.23599 \\
8 7.3787400000000005 \\
9 8.53679 \\
10 9.87391 \\
11 11.21596 \\
12 12.606630000000001 \\
13 14.198310000000001 \\
14 15.874390000000002 \\
15 17.56284 \\
16 19.270880000000002 \\
17 21.01745 \\
18 22.803350000000002 \\
19 24.616950000000003 \\
20 26.57345 \\
21 28.81068 \\
22 31.95024 \\
23 36.34177 \\
24 42.10816 \\
25 48.882909999999995 \\
26 56.56455999999999 \\
27 64.35291 \\
28 73.37728999999999 \\
29 82.55286999999998 \\
30 94.75292999999999 \\
31 107.29166 \\
32 123.30492 \\
33 146.91953 \\
34 179.59788 \\
35 221.98718 \\
36 274.56542 \\
37 330.76075000000003 \\
38 387.22477000000003 \\
39 444.12682000000007 \\
40 501.8145600000001 \\
41 571.4382700000001 \\
42 643.4474000000001 \\
43 722.4194800000001 \\
44 821.2283400000001 \\
45 929.1789600000001 \\
46 1052.78297 \\
47 1189.84376 \\
48 1341.92238 \\
49 1497.50966 \\
50 1682.04275 \\
51 1874.04086 \\
52 2097.30546 \\
53 2354.25167 \\
54 2614.46702 \\
55 2882.47859 \\
56 3160.20235 \\
57 3509.9588400000002 \\
58 3898.5201700000002 \\
59 4310.69438 \\
60 4878.89952 \\
61 5475.02516 \\
62 6071.41619 \\
63 6733.51141 \\
64 7500.94068 \\
65 8435.01191 \\
66 10161.85311 \\
};

\addplot+ [
sharp plot,
color=rred,
solid, thick,
mark=none,
] table[
row sep=\\]{
0 0.1 \\
1 0.40179000000000004 \\
2 0.8937200000000001 \\
3 1.48462 \\
4 2.13582 \\
5 2.9084399999999997 \\
6 3.7332599999999996 \\
7 4.566339999999999 \\
8 5.4378899999999994 \\
9 6.498939999999999 \\
10 7.574339999999999 \\
11 8.68561 \\
12 9.796940000000001 \\
13 10.90848 \\
14 12.109750000000002 \\
15 13.710990000000002 \\
16 15.342290000000002 \\
17 17.273970000000002 \\
18 19.587030000000002 \\
19 22.07832 \\
20 24.659380000000002 \\
21 27.251340000000003 \\
22 30.532420000000002 \\
23 34.3134 \\
24 38.4345 \\
25 43.08578 \\
26 47.8776 \\
27 52.68873 \\
28 57.61007 \\
29 64.39117 \\
30 73.47800000000001 \\
31 84.73185000000001 \\
32 96.46279000000001 \\
33 108.27511000000001 \\
34 122.49651000000001 \\
35 141.04812 \\
36 159.99996000000002 \\
37 179.07191 \\
38 201.87386 \\
39 229.23783 \\
40 257.87441 \\
41 289.49636000000004 \\
42 321.85623000000004 \\
43 354.67783000000003 \\
44 392.54888000000005 \\
45 432.1220400000001 \\
46 471.7430100000001 \\
47 512.29556 \\
48 562.3478 \\
49 617.40896 \\
50 673.7326499999999 \\
51 740.96597 \\
52 811.80011 \\
53 895.53317 \\
54 996.6199300000001 \\
55 1104.54693 \\
56 1225.60804 \\
57 1347.7017500000002 \\
58 1531.2447300000001 \\
59 1762.7796700000001 \\
60 2041.3813 \\
61 2361.80254 \\
62 2694.42371 \\
63 3073.28639 \\
64 3513.15171 \\
65 4229.31308 \\
66 5558.90575 \\
};

\addplot+ [
sharp plot,
color=ggreen,
solid, thick,
mark=none,
] table[
row sep=\\]{
0 0.1 \\
1 4.18001 \\
2 18.76979 \\
3 33.46673 \\
4 49.38339 \\
5 65.65704 \\
6 82.18593999999999 \\
7 101.01029999999999 \\
8 119.93104999999998 \\
9 154.67158999999998 \\
10 190.39051999999998 \\
11 247.26144999999997 \\
12 327.07119 \\
13 516.6460500000001 \\
14 799.7217600000001 \\
15 1165.4522100000002 \\
16 1549.2283000000002 \\
17 1944.0775900000003 \\
18 2341.0765900000006 \\
19 2789.6372600000004 \\
20 3242.7000900000003 \\
21 3755.45733 \\
22 4284.7671 \\
23 4814.13043 \\
24 5344.41562 \\
25 5887.4403 \\
26 6445.208860000001 \\
27 7095.474580000001 \\
28 7899.148390000001 \\
29 8767.792590000001 \\
30 9735.54723 \\
31 10817.79832 \\
32 12040.67903 \\
33 13289.380079999999 \\
34 15838.46856 \\
};

\end{axis}
\end{tikzpicture}


==> figures/comparisons/legend.tex <==
\begin{tikzpicture}[scale=0.5, transform shape]
    \begin{customlegend}[legend entries={Folding,Labyrinth,Rubik's Cube,Slitherlink, Quantum, Recharging, Ricochet}, legend columns=4, legend style={draw=none, font=\scriptsize}]
        %\addlegendimage{mark=*, mark size=2pt}
        %\addlegendimage{mark=square*, mark size=2pt}
        \addlegendimage{gray, mark=triangle*, mark size=2pt}
        \addlegendimage{gray, mark=diamond*, mark size=2pt}
        \addlegendimage{gray, mark=Mercedes star, mark size=2.5pt}
        \addlegendimage{gray, mark=halfcircle*, mark size=2pt}
        \addlegendimage{gray, mark=pentagon*, mark size=2pt}
        \addlegendimage{gray, mark=heart, mark size=2pt}
        \addlegendimage{gray, mark=halfdiamond*, mark size=2pt}
    \end{customlegend}
\end{tikzpicture}

==> figures/comparisons/symk_time_grd.tex <==
\begin{tikzpicture}[scale=0.88]
\begin{axis}[
    xmode=log,
    ymode=log,
   xlabel={Run Time \lcc + \symk\ (sec)},
   ylabel={Run Time \lccr + \symk\ (sec)},
    title = Ground Constraints, 
    width=5.4cm,
    height=5.4cm,
    grid=none,
    mark size=2pt,
    xmin=0.11,
    ymin=0.11,
    xmax=2000,
    ymax=2000,
     xlabel style={yshift=3pt},
     ylabel style={yshift=-3pt},
     title style={yshift=-5pt},
     font=\footnotesize,
]

\addplot [black, dashed, domain=0.001:1800, forget plot] {x};

\addplot+ [
only marks,
mark=triangle*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=diamond*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
45.3434 59.484140000000004 \\
0.96319 0.76415 \\
0.893 0.735 \\
1.02289 0.72359 \\
0.45275 0.47497 \\
0.63319 0.67996 \\
41.882560000000005 82.04015000000001 \\
92.08335 52.50092 \\
100.07314 74.81066 \\
403.90765999999996 253.51891 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=pentagon*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
3.2816199999999998 2.7736099999999997 \\
35.621539999999996 54.76218 \\
295.11142 284.2599 \\
1800 1800 \\
388.35189 344.96909999999997 \\
1365.5017 1245.84962 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
6.10085 9.98846 \\
43.38256 57.63502 \\
329.28376 360.08696000000003 \\
638.24442 721.88697 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=heart,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
0.85156 0.53448 \\
2.77104 1.9282199999999998 \\
5.7212 14.06554 \\
7.0718000000000005 18.46708 \\
0.6711900000000001 1.1194899999999999 \\
0.52088 0.5153 \\
5.32102 2.34659 \\
2.0511899999999996 1.92107 \\
0.9214800000000001 0.81732 \\
7.28104 2.5328600000000003 \\
1.9310399999999999 1.71019 \\
48.07096 177.26674 \\
10.98103 36.16202 \\
5.41101 5.41493 \\
41.60087 48.49841 \\
94.88100999999999 322.30012999999997 \\
3.77083 3.99988 \\
842.1808699999999 834.25631 \\
144.06157 38.403389999999995 \\
1800 506.25081 \\
};

\addplot+ [
only marks,
mark=halfdiamond*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
0.43139 0.41979 \\
3.79092 10.09724 \\
0.51092 0.47868999999999995 \\
2.27091 16.07678 \\
12.75112 5.14658 \\
12.70112 6.16286 \\
8.68094 25.02942 \\
31.29109 79.81394999999999 \\
2.42111 2.83262 \\
44.191649999999996 103.36219 \\
103.72111 82.88255000000001 \\
10.7714 7.15721 \\
11.450949999999999 20.27845 \\
13.76121 8.84716 \\
36.44114 23.522810000000003 \\
23.89097 39.39937 \\
13.90093 13.80864 \\
41.86094 24.523310000000002 \\
95.76093 45.7083 \\
32.17096 30.41123 \\
};

\addplot+ [
only marks,
mark=Mercedes star,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
1800 1800 \\
1800 1800 \\
936.0565799999999 928.69409 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=halfcircle*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
0.50195 4.26504 \\
0.7917500000000001 1.1071 \\
2.51171 2.83235 \\
2.4417 2.47272 \\
1.1215600000000001 3.8963300000000003 \\
2.40179 3.1231 \\
2.76177 3.663 \\
36.311710000000005 42.87041000000001 \\
44.29173 39.81925 \\
44.2023 38.82695 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\end{axis}
\end{tikzpicture}


==> figures/comparisons/symk_time_lfd.tex <==
\begin{tikzpicture}[scale=0.88]
\begin{axis}[
    xmode=log,
    ymode=log,
    xlabel={Run Time \lcc\ + \symk\ (sec)},
    %ylabel={Execution Time LCCR + SYMK (sec)},
    yticklabels={},
    title = Non-Ground Constraints,
    width=5.4cm,
    height=5.4cm,
    grid=none,
    mark size=2pt,
    xmin=0.11,
    ymin=0.11,
    xmax=2000,
    ymax=2000,
     xlabel style={yshift=3pt},
     ylabel style={yshift=-3pt},
     title style={yshift=-5pt},
     font=\footnotesize,
]

\addplot [black, dashed, domain=0.001:1800, forget plot] {x};

\addplot+ [
only marks,
mark=triangle*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1.60124 1.34205 \\
1.1112700000000002 1.02989 \\
14.221400000000001 2.2372300000000003 \\
1.6313 1.33712 \\
1.1113300000000002 1.09712 \\
1800 1800 \\
4.8111299999999995 1.68845 \\
4.1211 1.8136 \\
2.4912900000000002 1.7859 \\
4.92134 1.74657 \\
2.58106 1.9565 \\
4.651280000000001 1.70804 \\
1.20127 1.1427500000000002 \\
};

\addplot+ [
only marks,
mark=diamond*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
83.73306000000001 107.95062 \\
0.77262 0.90945 \\
0.8330799999999999 1.59168 \\
0.82482 1.07271 \\
2.31306 1.15805 \\
1.0754000000000001 5.7663899999999995 \\
122.09371 155.58728000000002 \\
183.54298 137.06079 \\
1800 767.42927 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=pentagon*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
4.79182 7.788349999999999 \\
716.1613699999999 596.12564 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
27.36397 56.46402 \\
1329.59267 934.07123 \\
231.53494 268.01157 \\
439.86532 412.17421 \\
1800 1800 \\
1800 1726.8411999999998 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=heart,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
1800 1800 \\
1800 1800 \\
0.87155 1.39067 \\
55.06116 277.72375999999997 \\
1.06105 16.013260000000002 \\
1800 1800 \\
37.87105 184.53309000000002 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
32.821600000000004 12.20006 \\
6.7811 4.3915299999999995 \\
1800 1800 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=halfdiamond*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
0.40179000000000004 0.5508700000000001 \\
3.78098 12.53873 \\
0.6512 1.0678100000000001 \\
3.2810799999999998 7.68165 \\
121.06111 23.614610000000003 \\
0.5909 1.67608 \\
11.73094 56.90205 \\
18.55161 72.00913 \\
11.25385 9.02438 \\
332.62117 349.75649 \\
39.62097 78.97208 \\
40.55255 56.19533 \\
22.80195 388.56133 \\
28.63658 42.3893 \\
378.86268 568.20514 \\
32.35987 596.39103 \\
39.57316 57.68774 \\
31.621950000000002 152.07862 \\
278.60163 223.2646 \\
320.42124 662.09522 \\
};

\addplot+ [
only marks,
mark=Mercedes star,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
1800 1800 \\
107.927 123.60401 \\
1800 1800 \\
1800 1800 \\
101.08676 98.80886000000001 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\addplot+ [
only marks,
mark=halfcircle*,
mark options={solid,draw=gray,fill=gray},
] table[
row sep=\\]{
0.49193 0.50814 \\
1.1115400000000002 6.77475 \\
1.9316799999999998 32.67835 \\
1800 1800 \\
9.08683 3.1395600000000004 \\
2.59196 9.17558 \\
19.07195 1800 \\
18.95184 256.94621 \\
11.81232 1800 \\
1800 1800 \\
50.05224 52.57824 \\
56.32369 69.62371 \\
1800 1800 \\
67.23332 191.99811 \\
70.83414 260.21535 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
1800 1800 \\
};

\end{axis}
\end{tikzpicture}

